F1 is Not Enough! Models and Evaluation Towards User-Centered Explainable Question Answering

Explainable question answering systems predict an answer together with an explanation showing why the answer has been selected. The goal is to enable users to assess the correctness of the system and understand its reasoning process. However, we show that current models and evaluation settings have shortcomings regarding the coupling of answer and explanation which might cause serious issues in user experience. As a remedy, we propose a hierarchical model and a new regularization term to strengthen the answer-explanation coupling as well as two evaluation scores to quantify the coupling. We conduct experiments on the HOTPOTQA benchmark data set and perform a user study. The user study shows that our models increase the ability of the users to judge the correctness of the system and that scores like F1 are not enough to estimate the usefulness of a model in a practical setting with human users. Our scores are better aligned with user experience, making them promising candidates for model selection.

==> sections/analysis.tex <==
In this section, we detail the task we address in this paper and present limitations of existing models and evaluation settings.

\subsection{Task}
In our setting, explainable question answering (XQA) is the task of (\romannum{1}) answering a question and (\romannum{2}) providing an explanation that enables the user to understand \textit{why} the answer was selected.
Importantly, this also includes to adequately explain \textit{wrong} answers.
To detail the task we consider in this paper, the selection of an answer corresponds to  selecting ``yes'', ``no'' or a text span from the context that is available to the model while predicting an explanation corresponds to selecting the set of relevant sentences from that context. The explanation sentences should be as precise as possible, i.e., including all the information necessary to follow the reasoning chain of the model and at the same time not including additional superfluous information.

\subsection{Limitations of Current Evaluation}
Current evaluation of XQA is focused on three scores: (\romannum{1}) answer-\F\ , which is based on the token overlap between the predicted and the ground truth answer, (\romannum{2}) SP-\F\ , which calculates \F\ based on the overlap of predicted and ground truth relevant facts and (\romannum{3}) joint-\F\ , which is based on the definitions of joint recall and joint precision as the products of answer and SP recall and precision.
The \textsc{HotpotQA} leaderboard ranks model submissions based on joint-\F\ , making it the defacto standard for XQA evaluation.
We argue that this undermines the development of truly usable XQA models for the following reasons:
\paragraph{No Empirical Evidence}
There is no empirical evidence that joint-\F\ is relates to user performance or experience regarding XQA at all.
\paragraph{Rewarding Poor Explanations}
Figure~\ref{fig:motivating_example} shows an example prediction that is rewarded with a joint-\F\ of 0.5 although its explanation provides no value to the user.
The reward stems from the overlap of the explanation with the ground truth and reveals the more fundamental problem of relying on ground truth data for explanations, which becomes even clearer for the next problem.
\paragraph{Punishing Good Explanations}
Figure~\ref{fig:zero_f1_good_explanation}.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/drawn/teaser 2.pdf}
    \caption{Correct example prediction that is assigned zero for all \F-scores because there is a second football club in Lesotho to which the ground truth annotation refers to. \textcolor{green}{(bold face answer in fact as in first figure)}}
    \label{fig:zero_f1_good_explanation}
\end{figure}
The prediction shown in Figure~\ref{fig:zero_f1_good_explanation} shows an explanation that receives a joint-\F\ although it is perfectly correct.
This paradox situation is caused by the fact that there are also is the ``Lerotholi Polytechnic Football Club'' in Lesotho and the annotator did (correctly) annotate the answer and explanation with respect to that club and not with respect to ``Matlama FC''.
This example highlights that exclusively relying on ground truth explanations can be counterproductive.


We want to emphasize that our goal is not to belittle work that has been done on improving joint-\F\ .
Among all standard scores we agree that \F~is the most intuitive and best-suited one to capture XQA performance.
However, we argue that it is time to consider whether the direction we aim at also is the right one and to re-adjust our objectives in order to target work that makes a difference for humans.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/drawn/baseline_abstract.pdf}
    \caption{Abstract architecture of the baseline models.}
    \label{fig:bl_architecture}
\end{figure}

\textcolor{blue}{
}

\subsection{Limitations of Current Models}\label{sec:weaknesses}
We manually review model predictions of the model by \newcite{qi2019answering} and identify two problems regarding answer-explanation coupling.
First, the model makes use of facts without including them into its explanations.
\textcolor{blue}{\st{Table~1}(removed table) Figure~\ref{fig:motivating_example}} shows an example of this \textit{silent integration} of facts.
The predicted answer does not occur in the relevant facts (i.e., the explanation).
Thus the user does not know where it comes from.

Second, the model predicts facts to be relevant without any comprehensible relation to the predicted answer.
An example of such \textit{unused facts} is shown in \textcolor{blue}{\st{}Table~2}(replaced table with Figure) Figure~\ref{fig:unused_facts}.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/drawn/teaser 4.pdf}
    \caption{Example of unused facts predicted to be relevant. The last (red-colored) fact is irrelevant to the human reasoning process (prediction of the baseline model).}\label{tab:example_no_usage}
    \label{fig:unused_facts}
\end{figure}

\textcolor{red}{TODO: say why this happens: no explicit coupling in model of explanations and answers; independent heads and loss function terms; say that this is also true for other SOA models in XQA and cite some of them as examples}
\textcolor{green}{$\Rightarrow$ added paragraph below. We can't really claim that this also happens for SOA models, but we can make a generalization over the used BiDaf++ architecture as it is used in at least four models on \textsc{HotpotQA} and can be regarded to be the largest similarity among all models, which }

The examples shed light on a lack of coupling between the answer and the explanation.

